SeedFold: Scaling Biomolecular Structure Prediction

Highly accurate biomolecular structure prediction is a key component of developing biomolecular foundation models, and one of the most critical aspects of building foundation models is identifying the recipes for scaling the model. In this work, we present SeedFold, a folding model that successfully scales up the model capacity. Our contributions are threefold: first, we identify an effective width-scaling strategy for the Pairformer to increase representation capacity; second, we introduce a novel linear triangular attention that reduces computational complexity to enable efficient scaling; finally, we construct a large-scale distillation dataset to substantially enlarge the training set. Experiments on FoldBench show that SeedFold outperforms AlphaFold3 on most protein-related tasks.

==> tables/ablation.tex <==
% Ablation table for SeedFold
\begin{table}[h]
\centering
\caption{Leave-One-Out Ablations on 384-width SeedFold}
\label{tab:leave-one-out_ablation}
\begin{tabular}{l cc}
\toprule
\textbf{Setting} & \textbf{Protein (LDDT)} & \textbf{Prot-Prot (DockQ)}\\
\midrule
SeedFold (Full) & -- & -- \\
\midrule
\ \ w/o Linear Triangular Attention & -- & -- \\
\ \ w/o MSA Module Expansion & -- & -- \\
\ \ w/o Large-Scale Distillation & -- & -- \\
\ \ w/o Two-Stage Training & -- & -- \\
\bottomrule
\end{tabular}%
\end{table}


==> tables/incremental.tex <==
% Incremental results table for SeedFold
\setcounter{table}{0}
\begin{table}[t]
    \centering
    \caption{Incremental improvements from scaling and data strategies}
    \begin{tabular}{l ccc}
        \toprule
        \textbf{Configuration} & \textbf{Protein (LDDT)} & \textbf{Prot-Prot (DockQ)} & \textbf{Prot-Lig (SR\%)} \\
        \midrule
        \textbf{AlphaFold 3} & 0.88 & 72.9\% & 64.9\% \\
        \midrule
        Base (128-width, PDB only) & -- & -- & -- \\
        + Large-Scale Distillation & -- & -- & -- \\
        + Width Scaling (256) & -- & -- & -- \\
        + Width Scaling (384) & -- & -- & -- \\
        + Linear Triangular Attention & -- & -- & -- \\
        + Two-Stage Training (\textbf{SeedFold}) & \textbf{--} & \textbf{--} & \textbf{--} \\
        \bottomrule
    \end{tabular}
    \label{tab:incremental_results}
\end{table}

